"It depends": Configuring AI to Improve Clinical Usefulness Across Contexts

Artificial Intelligence (AI) repeatedly match or outperform radiologists in lab experiments. However, real-world implementations of radiological AI-based systems are found to provide little to no clinical value. This paper explores how to design AI for clinical usefulness in different contexts. We conducted 19 design sessions and design interventions with 13 radiologists from 7 clinical sites in Denmark and Kenya, based on three iterations of a functional AI-based prototype. Ten sociotechnical dependencies were identified as crucial for the design of AI in radiology. We conceptualised four technical dimensions that must be configured to the intended clinical context of use: AI functionality, AI medical focus, AI decision threshold, and AI Explainability. We present four design recommendations on how to address dependencies pertaining to the medical knowledge, clinic type, user expertise level, patient context, and user situation that condition the configuration of these technical dimensions.

==> content/NOTES.tex <==
Jorge to have a look at: 

- Format of the findings, highlighting parts that are unclear, parts that seem extra and could be deleted. (just a high level review, I'll be still working on it but as a sanity check)

- Give it a try in describing the prototypes and proposing images from the design interventions. Screenshots of the prototype. 


The second/third main iteration of the prototype consisted of an interactive web application designed to emulate a DICOM viewer. The web application integrated with the AI system that was being developed, which enabled us to work with real data, and thus, explore with fidelity the interactions of the radiologists with the system. For the design interventions, radiologist were given access to the prototype, either in-person or remotely. They were requested to perform some tasks, but were free to explore the prototype on their own and interact with any element on the user interface.

The development of this prototype when through an interactive process, and incremental improvements to the prototype were made with the feedback collected from radiologists after each intervention. In the prototype, we explored three main aspects of interest for the development of an AI medical system: 1) the prioritisation of cases, 2) the explainability and visualization of AI findings and 3) the configuration of the system. 
